Interval centred form for proving stability of non-linear discrete-time systems

In this paper, we propose a new approach to prove stability of non-linear discrete-time systems. After introducing the new concept of stability contractor, we show that the interval centred form plays a fundamental role in this context and makes it possible to easily prove asymptotic stability of a discrete system. Then, we illustrate the principle of our approach through theoretical examples. Finally, we provide two practical examples using our method : proving stability of a localisation system and that of the trajectory of a robot.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{T. Dang and S. Ratschan: 6th International Workshop on\\Symbolic-Numeric Methods for Reasoning about CPS and IoT (SNR 2020)\\
EPTCS 331, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.331.1}{10.4204/EPTCS.331.1}}
\pdfoutput=1

